Optimal inference for the mean of random functions

We study estimation and inference for the mean of real-valued random functions defined on a hypercube. The independent random functions are observed on a discrete, random subset of design points, possibly with heteroscedastic noise. We propose a novel optimal-rate estimator based on Fourier series expansions and establish a sharp non-asymptotic error bound in $L^2-$norm. Additionally, we derive a non-asymptotic Gaussian approximation bound for our estimated Fourier coefficients. Pointwise and uniform confidence sets are constructed. Our approach is made adaptive by a plug-in estimator for the H\"older regularity of the mean function, for which we derive non-asymptotic concentration bounds.

==> sections/SM_sum_sin_cos.tex <==
% !TeX root = ../mean_SM.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% The working version as created by Valentin Jan 12
%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{lemma}\label{sum_sin_cos}
	For $\mathbf t \in \mathcal T$ and $L\in \mathbb N$, let
	$$\theta (L, D)= \sum_{ | \mathbf k|_1 \leq 2L } \phi_{\mathbf k} ^2(\mathbf t).$$ 
	Then, for any $\mathbf t \in \mathcal T$, we have 
	\begin{equation}
		\frac{1}{L} \sum_{j=0}^{L-1}\theta (L+j, D) = \frac{2^{2D+1} -2^D}{ (D+1)!} L^D + O(L^{D-1}) = \frac{2^{2D+1} -2^D}{ (D+1)!} L^D\{1+o(1)\},
	\end{equation}
	and the constants in the terms $O(L^{D-1})$ and $o(1)$ do not depend on $\mathbf t$.
\end{lemma}

\medskip

\begin{proof}[Proof of Lemma \ref{sum_sin_cos}]
	Let $J \in \mathbb N$, we have 
	\begin{multline}
		\theta (J, D)=\sum_{ | \mathbf k|_1 \leq 2J } \phi_{\mathbf k} ^2(\mathbf t) = 1 + \sum_{\ell=1}^{ 2J} \sum_{ \{k_1+ k_2 + \dots + k_D = \ell\}}\prod _{j=1}^D \phi_{ k_j} ^2(t_j)\\
			= 1 + \sum_{\ell=1}^{ J}\left\{ \sum_{ k_1= 0}^{ 2\ell}\sum_{ \{ k_2 + \dots + k_D = 2\ell -k_1\}}\prod _{j=1}^D \phi_{ k_j} ^2(t_j) +  \sum_{ k_1= 0}^{ 2\ell- 1}\sum_{  \{k_2 + \dots + k_D = (2\ell -1) -k_1\}}\prod _{j=1}^D \phi_{ k_j} ^2(t_j)\right\}\\
		\hspace{-7.6cm}= 1 + \underbrace{\sum_{\ell=1}^{ 2J} \sum_{  \{k_2 + \dots + k_D = \ell\}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j)}_{\beta(J,D-1)}\\
			\quad \quad + \sum_{\ell=1}^{ J} \left\{\sum_{ k_1= 1}^{ 2\ell}\sum_{ \{ k_2 + \dots + k_D = 2\ell -k_1\}}\prod _{j=1}^D \phi_{ k_j} ^2(t_j) +  \sum_{ k_1= 1}^{ 2\ell- 1}\sum_{  \{k_2 + \dots + k_D = (2\ell -1) -k_1\}}\prod _{j=1}^D \phi_{ k_j} ^2(t_j)\right\}\\
		\hspace{-10.7cm} = : 1 + \beta (J, D-1)
		%\sum_{\ell=1}^{ 2J} \sum_{  k_2 + \dots + k_D = \ell}\prod _{i=2}^D \phi_{ k_j} ^2(t_j)
		\\
		+ \sum_{\ell=1}^{ J} \sum_{ k_1=1}^{ \ell}\left\{\sum_{\{  k_2 + \dots + k_D = 2\ell -2k_1\}} \phi_{2k_1}^2(t_1) \prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right.\\ \hspace{4.2cm}\left. + \sum_{  \{k_2 + \dots + k_D = 2\ell -(2k_1-1)\}} \phi_{2k_1 -1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right\} \\
		+  \sum_{\ell=1}^{ J}\left\{ \sum_{ k_1= 1}^{ \ell-1}\sum_{  \{k_2 + \dots + k_D = (2\ell -1) -2k_1\}} \phi_{2k_1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \right.\\ \hspace{6cm}\left. +\sum_{ k_1= 1}^{ \ell}\sum_{ \{ k_2 + \dots + k_D = (2\ell-1)  -(2k_1-1)\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right\}	.	
	\end{multline}		
Grouping terms and using the fact that $\phi_{2k_1-1}^2(t_1)+\phi_{2k_1}^2(t_1)=2$, 
we get		
		\begin{multline}	
		\theta (J, D)= 1 
		%+\sum_{\ell=1}^{ 2J} \sum_{  k_2 + \dots + k_D = \ell}\prod _{i=2}^D \phi_{ k_j} ^2(t_j)
		+\beta (J, D-1)
		+2\sum_{\ell=1}^{ J} \sum_{ k_1= 1}^{ \ell}\sum_{\{  k_2 + \dots + k_D = 2\ell -2k_1\}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \\
		+\sum_{\ell=1}^{ J}  \left\{\sum_{ k_1= 1}^{ \ell-1}\sum_{  \{k_2 + \dots + k_D = 2\ell-2k_1-1\}} \phi_{2k_1}^2(t_1)\prod _{i=2}^D \phi_{ k_j} ^2(t_j)\right.\\ \hspace{8cm}\left.+\sum_{ k_1= 1}^{ \ell}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{i=2}^D \phi_{ k_j} ^2(t_j)\right\}\\
		=: 1	+\beta (J, D-1)+ 		2\sum_{\ell=1}^{ J} \sum_{ k_1= 1}^{ \ell}\sum_{\{  k_2 + \dots + k_D = 2\ell -2k_1\}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j) + S(J).
	\end{multline}
	Using Fubini for the last sums, we can write,	
	\begin{multline}
	%	\sum_{\ell=1}^{ J}  \left\{\sum_{ k_1= 1}^{ \ell-1}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1-1\}} \phi_{2k_1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right.\\ \hspace{4cm}\left. +\sum_{ k_1= 1}^{ \ell}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right\}\\
	S(J)	= \sum_{k_1= 1}^{J-1}\sum_{\ell=k_1+1 }^J\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1-1\}} \phi_{2k_1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \\
			\hspace{4cm}+ \sum_{k_1= 1}^{J} \sum_{\ell=k_1 }^J\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\\
	\stackrel{\ell^\prime = \ell+1}{=}	 \sum_{k_1= 1}^{J-1}\sum_{\ell^\prime=k_1 }^{J-1}\sum_{  \{k_2 + \dots + k_D = 2\ell^\prime  -2k_1+1\}} \phi_{2k_1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \\
		\hspace{4cm}+ \sum_{k_1= 1}^{J} \sum_{\ell=k_1 }^J\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\\
		= \sum_{k_1= 1}^{J-1}\sum_{\ell^\prime=k_1 }^{J-1}\sum_{  \{k_2 + \dots + k_D = 2\ell^\prime +1 -2k_1\}} \phi_{2k_1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \\
		\hspace{4cm}+ \sum_{k_1= 1}^{J-1} \sum_{\ell=k_1 }^{J-1}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\\
		\hspace{5cm}+ \sum_{k_1= 1}^{J} \sum_{  \{k_2 + \dots + k_D = 2J -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \\
	\stackrel{\phi_{2k_1-1}^2(t_1)+\phi_{2k_1}^2(t_1)=2}{=}2 \sum_{k_1= 1}^{J-1} \sum_{\ell=k_1 }^{J-1}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \prod _{j=2}^D \phi_{ k_j} ^2(t_j)\\
		\hspace{4cm}+ \sum_{k_1= 1}^{J} \sum_{  \{k_2 + \dots + k_D = 2J -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j).
	\end{multline}
	Therefore, using again Fubini, the fact that $\phi_{2k_1-1}^2(t_1)=2- \phi_{2k_1}^2(t_1)$, we get
	\begin{multline}
		\theta (J, D ) 
		%\sum_{ | \mathbf k|_1 \leq 2J } \phi_{\mathbf k} ^2(\mathbf t) 
		=1 +  \beta (J, D-1)
	%	\\+\sum_{\ell=1}^{ 2J} \sum_{  k_2 + \dots + k_D = \ell}\prod _{j=2}^D \phi_{ k_j} ^2(t_j)
			\\+2\left\{\sum_{\ell=1}^{ J} \sum_{ k_1= 1}^{ \ell}\sum_{\{  k_2 + \dots + k_D = 2\ell -2k_1\}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j) 
			+\sum_{k_1= 1}^{J-1} \sum_{\ell=k_1 }^{J-1}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right\}
		\\+ \sum_{k_1= 1}^{J} \sum_{  \{k_2 + \dots + k_D = 2J -2k_1+1\}} \phi_{2k_1-1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\\
		\hspace{-9.2cm}= 1 + \beta (J, D-1)
		%\sum_{\ell=1}^{ 2J} \sum_{  k_2 + \dots + k_D = \ell}\prod _{j=2}^D \phi_{ k_j} ^2(t_j)
		\\	+2\left\{\sum_{\ell=1}^{ J} \sum_{ k_1= 1}^{ \ell}\sum_{\{  k_2 + \dots + k_D = 2\ell -2k_1\}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j) 
			+\sum_{\ell= 1}^{J} \sum_{k_1=1 }^{\ell}\sum_{  \{k_2 + \dots + k_D = 2\ell -2k_1+1\}} \prod _{j=2}^D \phi_{ k_j} ^2(t_j)\right\}
		\\+ \sum_{k_1= 1}^{J} \sum_{  \{k_2 + \dots + k_D = 2J -2k_1+1\}} (\phi_{2k_1-1}^2(t_1)-2)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\\
		=1+\beta (J, D-1)
	%	\underbrace{1 + \sum_{\ell=1}^{ 2J} \sum_{  k_2 + \dots + k_D = \ell}\prod _{j=2}^D \phi_{ k_j} ^2(t_j)}_{=O(J^{D-1})}
		+2\sum_{\ell=1}^{ J} \sum_{ k_1= 1}^{2 \ell}\sum_{\{  k_2 + \dots + k_D = 2\ell -k_1\}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j) \\
		- \underbrace{\sum_{k_1= 1}^{J} \sum_{  \{k_2 + \dots + k_D = 2J -2k_1+1\}} \phi_{2k_1}^2(t_1)\prod _{j=2}^D \phi_{ k_j} ^2(t_j)}_{=\gamma(J,D-1)}\\
		= 1+\beta (J, D-1)  + 2\sum_{\ell=1}^J \{\theta(\ell, D-1)- \delta(D-1)\} - \gamma(J,D-1),
	\end{multline}
	where 
	$$
	\delta(\ell, D-1) = \sum_{\{  k_2 + \dots + k_D = 2\ell  \}}\prod _{j=2}^D \phi_{ k_j} ^2(t_j)\lesssim \ell^{D-2},
	$$
		with the constant in $\lesssim$ depending only on $D$.
	Moreover, it is easy to notice that
	$$
\max\{ \beta (J, D-1),	\gamma(J,D-1), \theta(0, D-1)\}\lesssim J ^{D-1},
	$$
	with the constant in $\lesssim$ depending only on $D$.
	Therefore, we have 
	\begin{equation}
		\theta(J,D)= 2\sum_{\ell=0}^J \theta(\ell, D-1) + O(J^{D-1})= \left\{2\sum_{k_1=0}^J2 \sum_{k_2=0}^{k_1}\dots 2\sum_{k_D=0}^{k_{D-1}} 1\right\}+ O(J^{D-1}) .
	\end{equation}
	Faulhaber's formula, see \citet[ page 106]{Conway96}, gives  the coefficient of the largest power in the sum of positive powers. Thus
	\begin{equation}
		\theta(J,D)= \frac{2^{D}}{D!} J^D + O(J^{D-1}).
	\end{equation}
	The constant in the term $O(J^{D-1})$ does not depend on $\mathbf t$. 
	Thus, using Faulhaber's formula again, we get 
	\begin{multline}
		\frac{1}{L} \sum_{j=0}^{L-1}\theta (L+j, D) = \frac{2^{D}}{D! L}\sum_{j=0}^{L-1} (L+j)^D + O(L^{D-1})
	\\	= \frac{2^{D}}{D! L}\sum_{j=0}^{L-1}\sum_{k=0}^D \binom{D}{k} j^k L^{D-k} + O(L^{D-1})\\
		=  \frac{2^{D}}{D! L}\sum_{k=0}^D\binom{D}{k}  L^{D-k}\sum_{j=0}^{L-1} j^k + O(L^{D-1})
		\\\qquad = \frac{2^{D}}{D! L}\sum_{k=0}^D\frac{1}{k+1}\binom{D}{k}  L^{D-k}L^{k+1}+ O(L^{D-1})\\
		\quad =\frac{2^{D}}{D! }L^D \sum_{k=0}^D\frac{1}{D+1}\binom{D+1}{k+1}+ O(L^{D-1})
		\\=\frac{2^{D} ( 2^{D+1} -1)}{D!(D+1) }L^D + O(L^{D-1}).
	\end{multline}
	The constant in $O(L^{D-1})$ does not depend on $\mathbf t$. The proof  is now complete. \end{proof}





==> sections/discussion.tex <==
% !TeX root = ../mean.tex


\section{Discussion}\label{sec:disc}

*** TBC *** with a summary of what was done *** possible extensions ?
*** ETC

\subsection{Extensions}

here we are limited by the approximation theory. 

immediate extension via reflexion when $\alphamu \leq 1$.


*** why we restricted the class *** ? quote the other guys ***

\newpage

\subsection{Discussion}

Let us discuss in more detail the case $M_i\equiv 1$, which brings our problem of mean function inference to that of nonparametric inference for a standard regression function. One more time, the fact of considering random design matters.  First let us point that  standard approaches to constructing nonparametric confidence bands for functions are frustrated by the impact of bias. To overcome this problem it is common practice to either undersmooth, so as to reduce the impact of bias, or oversmooth, and thereby introduce an explicit or implicit bias estimator. As pointed in \cite{Was2008}, if $\widehat \mu(\mathbf t)$ is an estimator with mean $\mathbb E[ \widehat \mu(\mathbf t)]$ and standard diviation $\sqrt{\operatorname{Var} (\widehat \mu(\mathbf t))}$ then 
$$
\frac{\widehat \mu(\mathbf t)- \mu(\mathbf t)}{\sqrt{\operatorname{Var} (\widehat \mu(\mathbf t))}}=  \frac{\widehat \mu(\mathbf t)- \mathbb E[\widehat \mu(\mathbf t)]}{\sqrt{\operatorname{Var} (\widehat \mu(\mathbf t))}}+ \frac{\mathbb E[\widehat \mu(\mathbf t)]- \mu(\mathbf t)}{\sqrt{\operatorname{Var} (\widehat \mu(\mathbf t))}}.
$$
The first term typically satisfies a central limit theorem but the second term does not vanish even asymptotically if the bias and variance are balanced.






The proposition to use larger smoothing parameter $L^{\diamondsuit}$  in corollary \ref{coro_CB2} leads to smaller bias by oversmoothing, similar idea can be found in \citet[theorem 4.1]{zhou98} 

First, our inference is con
\begin{itemize}
	\item \cite{zhou98} see theorem 4.1,  ( fixed and random design)
	
	The under-smoothing of $\widehat \mu$ (by choosing $L= L^\diamondsuit$ ) to obtain confedence band centred at the mean function is possible under the knowledge  of $\alphamu$, if $M_i \equiv 1$ the estimated of the regularity in the next section does not converge since we ask for $M_i$ large enough 
	\item \cite{Low97}  Data-driven confidence bands that are simultaneously adaptive and honest do not exist for the class of Hölder functions
	
	
	
	\item \cite{Nickl2010} \cite{Nickl2016}Data-driven confidence bands that are simultaneously adaptive and honest do  exist for a large  subset of  the class of Hölder functions
	
	
\end{itemize}



\begin{remark}
	***TBC***	Note that, if $M_i = 1$ for any $1 \leq i \leq N$ and $L^* \asymp \log(N) N^{\frac{1}{2\alpha_\mu + D}}$, the average width of the resulting confidence band is of order $\log(N) N^{-\frac{\alpha_\mu}{2\alpha_\mu + D}}$, which matches the minimax rate of confidence bands for nonparametric regression functions (see \cite{CBadapt2014}). 
\end{remark}



\newpage


\subsection{Practical aspects}

*** put here ideas on the estimation of $f_{\mathbf T}$, $\sigma^2 (\cdot)$, $\gamma(\cdot,\cdot)$ if necessary !? ****

==> sections/subsampling.tex <==
% !TeX root = ../mean.tex




\subsection{Finite sample confidence bands by subsampling}
To construct confidence bands, we use a subsampling method that involves estimating the mean function using subsamples of the original dataset. This is an ensemble method, akin to the technique used for example  in Bagging; see \cite{buhlmann2012bagging} and \cite{buja2006observations}.  For any set $\mathcal S$, let $|\mathcal S|$ denote its cardinal. 
%Theoretical aspects of subsampling are discussed in \cite{politis1994} and related works.

Formally, let $\mathcal{E}^{\rm obs} = \{(i,m) : 1 \leq m \leq M_i, 1 \leq i \leq N\}$ denote the set of observed data indices. For a subset $\mathcal{A} \subset \mathcal{E}^{\rm obs}$, let $\widehat{\mu}^*(\cdot, \mathcal{A})$ be the estimated mean function constructed with the data $\{(Y_{i,m}, \mathbf{T}_{i,m}) : (i,m)  \in \mathcal{A}\}$ and the $L^*$ defined as in \eqref{L_general} with $|\mathcal A|$ instead of  $\overline M$ .
Furthermore, we denote by  $\mathcal{A}^{\rm subj}$ the subset of indices of the random functions with design points selected in the subsample $\mathcal{A}$  that is  $\mathcal{A}^{\rm subj} = \{1\leq i \leq N : \exists m \in \mathbb{N}^*, (i,m) \in \mathcal{A}\}$.
Moreover, for   $ i \in \mathcal A^{\rm subj}$, let $ \mathcal A^{\rm obj}(i)= \{ m\in \mathbb N^*: (i,m) \in \mathcal A\}$. We also define
$$
\Delta (\mathbf t, \mathcal{A}) =  \widehat{\mu}^{*}(\mathbf t, \mathcal A) -  \widehat{\mu}^{*}(\mathbf t)  , \qquad \Delta_{\infty}(\mathcal{A}) = %\sup_{\mathbf t \in \mathcal{T}} 
\left\| \widehat{\mu}^{*}(\cdot, \mathcal{A}) - \widehat{\mu}^{*}(\cdot)  \right\|_\infty,  
$$
and, for $\vartheta(|\mathcal A|) \geq 1$, let
$$
\tau_{\mathcal{A}} =\left(\vartheta(|\mathcal A|)  |\mathcal A|^{\frac{ \alphamu}{2\alphamu+D}}\right) \wedge \frac{ \sum_{ i \in \mathcal{A}^{\rm subj}} |\mathcal A^{\rm obj}(i)| }{  \sqrt{\sum_{ i \in \mathcal{A}^{\rm subj}} |\mathcal A^{\rm obj}(i)| (|\mathcal A^{\rm obj}(i)|  - 1)}}.
$$
By construction, $\tau_{\mathcal{E}^{obs}}$ is equal to $\min\{\vartheta(\overline M )r_1(L^*),r_2\}$ considered
in Corollary  \ref{coro_CB2}. Let $\mathcal{U}(z, \mathbf{t})$ and $\mathcal{U}_{\infty}(z)$ be the (non-asymptotic) CDFs of $\tau_{\mathcal{E}^{obs}} \Delta(\mathbf{t})$ and $\tau_{\mathcal{E}^{obs}} \Delta_{\infty}$, respectively. For  $\alpha \in (0,1)$, let
\begin{equation}
	c_N(\mathbf t, 1 - \alpha) = \inf\{ z : \mathcal{U}( z, \mathbf t) \geq 1 - \alpha\}, \qquad c_{N, \infty}(1 - \alpha) = \inf\{ z : \mathcal{U}_\infty( z) \geq 1 - \alpha\},
\end{equation}
be the associated  $(1 - \alpha)-$quantiles.
These CDFs and their quantiles can be approximated by subsampling. 

Following the findings in \cite{buja2006observations}, we consider subsamples $\mathcal A$ with  $|\mathcal A|=\lfloor \overline{M} / 2 \rfloor$. Let $N_s$ be the number of subsamples $\mathcal A$. For a fixed $z \in \mathbb{R}_+$, we uniformly draw $N_s$ subsets $\mathcal{A}_1, \dots, \mathcal{A}_{N_s} \subset \mathcal{E}^{obs}$ of size $\lfloor \overline{M} / 2 \rfloor$, and define:
\begin{equation}
	\widetilde {\mathcal U}( z,\mathbf  t) = \frac{1}{N_s} \sum_{1 \leq j \leq N_s} \mathbbm{1} \{\tau_{\mathcal{A}_j} \Delta(\mathbf t, \mathcal{A}_j) \leq z\} , \qquad \widetilde {\mathcal U}_\infty (z) = \frac{1}{N_s} \sum_{1 \leq j \leq N_s} \mathbbm{1}\{\tau_{\mathcal{A}_j} \Delta_\infty( \mathcal{A}_j) \leq z\} .
\end{equation}
For the theory it suffices to take $N_s = a N$ with some $a>0$. Note that the condition $\min \{r_1(L^*), r_2\}\rightarrow \infty$  implies $\tau_{\mathcal{A}}, N_s\rightarrow \infty$.  The estimated quantiles are then
\begin{equation}
	\widetilde c(\mathbf t, 1 - \alpha) = \inf\{ z :\widetilde  {\mathcal{U}}( z, \mathbf t) \geq 1 - \alpha\}, \qquad \widetilde  c_{\infty}(1 - \alpha) = \inf\{ z :\widetilde { \mathcal{U}}_\infty( z) \geq 1 - \alpha\}.
\end{equation}
Then, for any $\mathbf t \in \mathcal T$, our  pointwise confidence interval of level $(1-\alpha)$ is  
$$
CI(\mathbf t)=[\widehat{\mu}^{*}(\mathbf t) -\widetilde c(\mathbf t , 1 - \alpha/2)/ \tau_{\mathcal E^{obs}}\;,\;   \widehat{\mu}^{*}(\mathbf t)  -\widetilde c(\mathbf t, \alpha/2)/ \tau_{\mathcal E^{obs}} ].
$$
Moreover, the  uniform confidence band is given by the following lower and upper limits~:
$$
L(\mathbf t) = \widehat{\mu}^{*}(\mathbf t) -\widetilde  c_{ \infty}(1 - \alpha)/ \tau_{\mathcal E^{obs}}\quad \text{and} \quad U(\mathbf t) = \widehat{\mu}^{*}(\mathbf t) +\widetilde  c_{ \infty}(1 - \alpha)/ \tau_{\mathcal E^{obs}},\qquad \mathbf t \in\mathcal T.
$$
We adopt the notation from \cite{CBadapt2014} and write $CB=[L(\mathbf t), U(\mathbf t)]$. 
The validity of our confidence sets is stated below as a direct consequence of the non-asymptotic Gaussian approximation result in Theorem \ref{normal_approximation}, and the Corollaries \ref{coro_linear} and \ref{coro_CB}. The proof is omitted. 

\medskip

\begin{corollary}\label{cor_sub_samp}
	Assume that the conditions of Corollary \ref{coro_CB2} hold true, and $N_s = aN$ for some $a>0$. Then, for any $\mathbf{t}\in \mathcal{T} $,  if $\vartheta(|\mathcal A|) \rightarrow \infty$ or $r_2 \ll r_1(L^*)$, we have
	\begin{equation}
		\mathbb{P} \big( \mu( \mathbf{t}) \in CI(\mathbf{t}) \big)\rightarrow  1-\alpha
		\qquad \text{ and } \qquad 
		\mathbb{P} \big( \mu( \mathbf{s}) \in CB, \; \forall \mathbf{s} \in \mathcal{T} \big)\rightarrow 1-\alpha.
	\end{equation}
	If $\vartheta(|\mathcal A|) =1$ and $r_1(L^*)\lesssim r_2$, the  result remains true with $V_{L^*}(\mu;\cdot) $ replacing $\mu(\cdot)$.
\end{corollary}





==> sections/subsampling_SM.tex <==
% !TeX root = ../mean_SM.tex




\subsection{Finite sample confidence regions by subsampling}\label{subssampl_SM}

To construct confidence regions without estimating the matrix $\Sigma$, we use a subsampling method that involves estimating the mean function using subsamples of the original dataset. This is an ensemble method, akin to the technique used for example  in Bagging; see \cite{buhlmann2012bagging} and \cite{buja2006observations}.  For any set $\mathcal S$, let $|\mathcal S|$ denote its cardinal. 
%Theoretical aspects of subsampling are discussed in \cite{politis1994} and related works.

Formally, let $\mathcal{E}^{\rm obs} = \{(i,m) : 1 \leq m \leq M_i, 1 \leq i \leq N\}$ denote the set of observed data indices. For a subset $\mathcal{A} \subset \mathcal{E}^{\rm obs}$, let $\widehat{\mu}^*(\cdot, \mathcal{A})$ be the estimated mean function constructed with the data $\{(Y_{i,m}, \mathbf{T}_{i,m}) : (i,m)  \in \mathcal{A}\}$ and the $L^*$ defined as in \eqref{L_general} with $|\mathcal A|$ instead of  $\overline M$ .
Furthermore, we denote by  $\mathcal{A}^{\rm subj}$ the subset of indices of the random functions with design points selected in the subsample $\mathcal{A}$  that is  $\mathcal{A}^{\rm subj} = \{1\leq i \leq N : \exists m \in \mathbb{N}^*, (i,m) \in \mathcal{A}\}$.
Moreover, for   $ i \in \mathcal A^{\rm subj}$, let $ \mathcal A^{\rm obj}(i)= \{ m\in \mathbb N^*: (i,m) \in \mathcal A\}$. We also define
$$
\Delta (\mathbf t, \mathcal{A}) =  \widehat{\mu}^{*}(\mathbf t, \mathcal A) -  \widehat{\mu}^{*}(\mathbf t)  , \qquad \Delta_{\infty}(\mathcal{A}) = %\sup_{\mathbf t \in \mathcal{T}} 
\left\| \widehat{\mu}^{*}(\cdot, \mathcal{A}) - \widehat{\mu}^{*}(\cdot)  \right\|_\infty,  
$$
and, for $\vartheta(|\mathcal A|) \geq 1$, let
$$
\tau_{\mathcal{A}} =\left(\vartheta(|\mathcal A|)  |\mathcal A|^{\frac{ \alphamu}{2\alphamu+D}}\right) \wedge \frac{ \sum_{ i \in \mathcal{A}^{\rm subj}} |\mathcal A^{\rm obj}(i)| }{  \sqrt{\sum_{ i \in \mathcal{A}^{\rm subj}} |\mathcal A^{\rm obj}(i)| (|\mathcal A^{\rm obj}(i)|  - 1)}}.
$$
By construction, $\tau_{\mathcal{E}^{obs}}$ is equal to $\min\{\vartheta(\overline M )r_1(L^*),r_2\}$ considered
in Corollary  \ref{coro_CB2}. Let $\mathcal{U}(z, \mathbf{t})$ and $\mathcal{U}_{\infty}(z)$ be the (non-asymptotic) CDFs of $\tau_{\mathcal{E}^{obs}} \Delta(\mathbf{t})$ and $\tau_{\mathcal{E}^{obs}} \Delta_{\infty}$, respectively. For  $\alpha \in (0,1)$, let
\begin{equation}
	c_N(\mathbf t, 1 - \alpha) = \inf\{ z : \mathcal{U}( z, \mathbf t) \geq 1 - \alpha\}, \qquad c_{N, \infty}(1 - \alpha) = \inf\{ z : \mathcal{U}_\infty( z) \geq 1 - \alpha\},
\end{equation}
be the associated  $(1 - \alpha)-$quantiles.
These CDFs and their quantiles can be approximated by subsampling. 

Following the findings in \cite{buja2006observations}, we consider subsamples $\mathcal A$ with  $|\mathcal A|=\lfloor \overline{M} / 2 \rfloor$. Let $N_s$ be the number of subsamples $\mathcal A$. For a fixed $z \in \mathbb{R}_+$, we uniformly draw $N_s$ subsets $\mathcal{A}_1, \dots, \mathcal{A}_{N_s} \subset \mathcal{E}^{obs}$ of size $\lfloor \overline{M} / 2 \rfloor$, and define:
\begin{equation}
	\widetilde {\mathcal U}( z,\mathbf  t) = \frac{1}{N_s} \sum_{1 \leq j \leq N_s} \mathbbm{1} \{\tau_{\mathcal{A}_j} \Delta(\mathbf t, \mathcal{A}_j) \leq z\} , \qquad \widetilde {\mathcal U}_\infty (z) = \frac{1}{N_s} \sum_{1 \leq j \leq N_s} \mathbbm{1}\{\tau_{\mathcal{A}_j} \Delta_\infty( \mathcal{A}_j) \leq z\} .
\end{equation}
For the theory it suffices to take $N_s = a N$ with some $a>0$. Note that the condition $\min \{r_1(L^*), r_2\}\rightarrow \infty$  implies $\tau_{\mathcal{A}}, N_s\rightarrow \infty$.  The estimated quantiles are then
\begin{equation}
	\widetilde c(\mathbf t, 1 - \alpha) = \inf\{ z :\widetilde  {\mathcal{U}}( z, \mathbf t) \geq 1 - \alpha\}, \qquad \widetilde  c_{\infty}(1 - \alpha) = \inf\{ z :\widetilde { \mathcal{U}}_\infty( z) \geq 1 - \alpha\}.
\end{equation}
Then, for any $\mathbf t \in \mathcal T$, our  pointwise confidence interval of level $(1-\alpha)$ is  
$$
CI(\mathbf t)=[\widehat{\mu}^{*}(\mathbf t) -\widetilde c(\mathbf t , 1 - \alpha/2)/ \tau_{\mathcal E^{obs}}\;,\;   \widehat{\mu}^{*}(\mathbf t)  -\widetilde c(\mathbf t, \alpha/2)/ \tau_{\mathcal E^{obs}} ].
$$
Moreover, the  uniform confidence band is given by the following lower and upper limits~:
$$
L(\mathbf t) = \widehat{\mu}^{*}(\mathbf t) -\widetilde  c_{ \infty}(1 - \alpha)/ \tau_{\mathcal E^{obs}}\quad \text{and} \quad U(\mathbf t) = \widehat{\mu}^{*}(\mathbf t) +\widetilde  c_{ \infty}(1 - \alpha)/ \tau_{\mathcal E^{obs}},\qquad \mathbf t \in\mathcal T.
$$
We adopt the notation from \cite{CBadapt2014} and write $CB=[L(\mathbf t), U(\mathbf t)]$. 
In view of the non-asymptotic Gaussian approximation result in Theorem \ref{normal_approximation}, and the Corollaries \ref{coro_linear} and \ref{coro_CB}, below we conjecture the validity of our confidence sets. 
%The proof is omitted. 

\medskip

\begin{conjecture}\label{cor_sub_samp}
	Assume that the conditions of Corollary \ref{coro_CB2} hold true, and $N_s = aN$ for some $a>0$. Then, for any $\mathbf{t}\in \mathcal{T} $,  if $\vartheta(\overline M) \rightarrow \infty$ or $r_2 \ll r_1(L^*)$, we have
	\begin{equation}
		\mathbb{P} \big( \mu( \mathbf{t}) \in CI(\mathbf{t}) \big)\rightarrow  1-\alpha
		\qquad \text{ and } \qquad 
		\mathbb{P} \big( \mu( \mathbf{s}) \in CB, \; \forall \mathbf{s} \in \mathcal{T} \big)\rightarrow 1-\alpha.
	\end{equation}
	If $\vartheta(\overline M) =1$ and $r_1(L^*)\lesssim r_2$, we conjecture that the  result remains true with $V_{L^*}(\mu;\cdot) $ replacing $\mu(\cdot)$.
\end{conjecture}





==> sections/weights_march.tex <==
% !TeX root = ../mean_SM.tex





\section{The linear integration in the case $D=1$}\label{weights_sec1}

Below, we provide a refined investigation of the moments of the weights of the linear integration approach of \cite{leluc2024speeding} on the unit interval. 



\subsection{The expression of the weights for linear integration}\label{secB_weights}

Let us first provide some explicit formulae for $\widehat d_j$ and $\widehat c_j$ in the case of a generic, real-valued i.i.d. sample of design points $T_1,\ldots,T_n$. Let $S_l = T_{(l)}$, where $T_{(l)}$, $1\leq l \leq n$, is the $l-$th order statistics of the sample. Then, when $n\geq 5$, it is easy to see that 
\begin{multline}\label{dm_explicit}
	\widehat d_j	= \mathbbm{1}\{ (S_{j-2}+S_{j})/2\leq S_{j-1}\} \\ + \mathbbm{1}\{ S_{j+1}\leq (S_{j}+S_{j+2})/2\}  \in \{0,1,2\}, \quad \text{if }  3\leq j \leq n-2,
\end{multline}
\begin{equation}\label{dm_explicit_end_l}
	\widehat d_1	=  \mathbbm{1}\{ S_{2}\leq (S_{1}+S_{3})/2\}  \in \{0,1\}, \qquad 
	\widehat d_2	= 1 + \mathbbm{1}\{ S_{3}\leq (S_{2}+S_{4})/2\} \in \{1,2\},
\end{equation}
and 
\begin{multline}\label{dm_explicit_end_r}
	\widehat d_{n-1}	= 1 + \mathbbm{1}\{ S_{n-2}\geq (S_{n-3}+S_{n-1})/2\} \!\in \!\{1,2\} , \qquad \\ 
	\widehat d_{n}	= \mathbbm{1}\{ S_{n-1}\!\geq (S_{n-2}+S_{n})/2\} \! \in \!\{0,1\}.
\end{multline}
Meanwhile, in the case of uniform design points, 
\begin{multline}\label{cm_explicit}
	\widehat c_j	= (n-3) \frac{S_{j+1}-S_{j-1}}{2} + \frac{S_{j+1}-S_{j-2}}{2} +\frac{S_{j+2}-S_{j-1}}{2}\\
	= (n-2) \frac{S_{j+1}-S_{j-1}}{2} +\frac{S_{j+2}-S_{j-2}}{2}, \quad \text{if }  3\leq j \leq n-2,
\end{multline}
\begin{equation}\label{cm_explicit_l1}
	\widehat c_1	= (n-2) \frac{S_1+S_2}{2}	+  \frac{S_1+S_3}{2},
\end{equation}
\begin{equation}\label{cm_explicit_l2}
	\widehat c_2	= (n-3) \frac{S_{3}-S_{1}}{2} + \frac{S_{2}+S_{3}}{2} +\frac{S_{4}-S_{1}}{2} 
	=  (n-2) \frac{S_{3}-S_{1}}{2} +\frac{S_{2}+S_{4}}{2},
\end{equation}
and
\begin{multline}\label{cm_explicit_r1}
	\widehat c_{n-1}	= (n-3) \frac{S_{n}-S_{n-2}}{2} 	+  1  - \frac{S_{n-1}+S_{n-2}}{2}
	+  \frac{S_{n}-S_{n-3}}{2} \\
	= (n-2) \frac{S_{n}-S_{n-2}}{2} +  1- \frac{S_{n-1}+S_{n-3}}{2}
\end{multline}
\begin{equation}\label{cm_explicit_r2}
	\widehat c_{n}	= (n-2) \left[1- \frac{S_{n-1}+S_{n}}{2}\right] + 1-\frac{S_{n-2}+S_{n}}{2} .
\end{equation}

In the general case, if $F_T$ denotes the distribution function of $T$, we have
\begin{multline}\label{cm_explicit_nu}
	\widehat c_j	= (n-3)\left[F_T\left(\frac{S_{j}+S_{j+1}}{2}  \right) - F_T\left(\frac{S_{j-1}+S_{j}}{2}  \right) \right]\\
	+ \left[F_T\left(\frac{S_{j}+S_{j+1}}{2}  \right) - F_T\left(\frac{S_{j-2}+S_{j}}{2}  \right) \right]\\
	+ \left[F_T\left(\frac{S_{j}+S_{j+2}}{2}  \right) - F_T\left(\frac{S_{j-1}+S_{j}}{2}  \right) \right],  \quad \text{if }  3\leq j \leq n-2,
\end{multline}
\begin{equation}\label{cm_explicit_l1_nu}
	\widehat c_1	= (n-2)F_T\left(\frac{S_{1}+S_{2}}{2}\right) 	+  F_T\left(\frac{S_{1}+S_{3}}{2}\right) ,
\end{equation}
\begin{multline}\label{cm_explicit_l2_nu}
	\widehat c_2	= (n-3) \left[F_T\left(\frac{S_{2}+S_{3}}{2}  \right) - F_T\left(\frac{S_{1}+S_{2}}{2}  \right) \right] \\ + F_T\left(\frac{S_{2}+S_{3}}{2}  \right)   \\ +\left[F_T\left(\frac{S_{2}+S_{4}}{2}  \right) - F_T\left(\frac{S_{1}+S_{2}}{2}  \right) \right]\\
	=  (n-2) \left[F_T\left(\frac{S_{2}+S_{3}}{2}  \right) - F_T\left(\frac{S_{1}+S_{2}}{2}  \right) \right]  + F_T\left(\frac{S_{2}+S_{4}}{2}  \right) ,
\end{multline}
and
\begin{multline}\label{cm_explicit_r1_nu}
	\widehat c_{n-1}	= (n-3) \left[F_T\left(\frac{S_{n-1}+S_{n}}{2}  \right) - F_T\left(\frac{S_{n-2}+S_{n-1}}{2}  \right) \right] \\	+  \left[1- F_T\left(\frac{S_{n-2}+S_{n-1}}{2}  \right) \right]
\\	+  \left[F_T\left(\frac{S_{n-1}+S_{n}}{2}  \right) - F_T\left(\frac{S_{n-3}+S_{n-1}}{2}  \right) \right]  \\
	=(n-2) \left[F_T\left(\frac{S_{n-1}+S_{n}}{2}  \right) - F_T\left(\frac{S_{n-2}+S_{n-1}}{2}  \right) \right] \\	+  \left[1- F_T\left(\frac{S_{n-3}+S_{n-1}}{2}  \right) \right],
\end{multline}
\begin{equation}\label{cm_explicit_r2_nu}
	\widehat c_{n}	= (n-2) \left[1- F_T\left(\frac{S_{n-1}+S_{n}}{2}  \right) \right] + 1-F_T\left(\frac{S_{n-2}+S_{n}}{2} \right).
\end{equation}


\subsection{The moments of the weights: uniform case}

In this section, we consider $S_1,\ldots,S_{n}$ to be the order statistics of a sample of independent uniform  variables on some interval $[a,b]$. In most statements, $[a,b] = [0,1]$.

\begin{lemma}\label{d1d2-lem}
	Let	$S_1,\ldots,S_{n}$ represent the order statistics of a uniform independent sample on $[a,b]$. 
	
	a) 	Let $3\leq j \leq n-2$. Then
	\begin{equation}\label{d1-lemma}
		\PP\left[(S_{j-2}+S_{j})/2\leq S_{j-1} \right] = \PP\left[S_{j+1}\leq (S_{j}+S_{j+2})/2 \right] = \frac{1}{2},
	\end{equation}
	and 
	\begin{equation}\label{d3-lemma}
		\PP\left[\{(S_{j-2}+S_{j})/2\leq S_{j-1} \}\cap \{S_{j+1}\leq (S_{j}+S_{j+2})/2 \}\right] = \frac{1}{4}.
	\end{equation}
	
	b) For $j \in\{1,2\}$ and $j^\prime  \in\{n-1,n\}$, 
	\begin{equation}\label{treez}
		\PP\left[S_{j+1} \leq (S_{j}+S_{j+2})/2  \right] = \frac{1}{2} = \PP\left[ (S_{j^\prime -2}+S_{j^\prime })/2 \leq S_{j^\prime -1}   \right].
	\end{equation}
\end{lemma}

\medskip

\begin{proof}[Proof of Lemma \ref{d1d2-lem}]
	Let us first note that, without loss of generality, we can consider $[a,b]=[0,1]$. This because, on the one hand, if $S_{1},\ldots, S_n$ is the order statistics of an independent uniform sample on $[a,b]$, then $U_j=(S_j - a )/(b-a)$, $1\leq j\leq n$, is the order statistics from an  independent uniform sample on $[0,1]$. On the other hand, the probabilities to be evaluated do not change if the $S_j$'s are replaced by the $U_j$'s. 
		
	a) First, consider $n=5$ and $j=3$. In this case, by direct calculations, we have
	\begin{multline}
		\PP\left[(S_{j-2}+S_{j})/2\leq S_{j-1} \right] \\ = 5! \int_{0 \leq t_1 \leq \dots \leq t_5 \leq 1} \mathbbm{1}\{t_2 \geq (t_3 + t_1)/2) \}dt_1 \dots dt_5 \\
		= 5! \int_{0 \leq t_2 \leq \dots \leq t_5 \leq 1} \int_{0}^{2t_2 - t_3} \mathbbm{1}\{2t_2 - t_3 > 0 \}  dt_1 dt_2 \dots dt_5 \\
		= 5! \int_{0 \leq t_2 \leq \dots \leq 1} (2t_2 - t_3) \mathbbm{1} \{2t_2 - t_3 > 0\} dt_2 \dots dt_5 \\
		= 5! \int_{0 \leq t_3 \leq \dots \leq 1}\int_{t_2 = t_3/2}^{t_3}   (2t_2 - t_3) dt_2 \dots dt_5 \\
		= 5! \int_{0 \leq t_4 \leq t_5 \leq 1} \int_{t_3 = 0}^{t_4}  \frac{t_3^2}{4} dt_3 dt_4 dt_5 \\
		= 5!\int_{0 \leq t_4 \leq t_5 \leq 1} \frac{t_4^3}{12} dt_4  dt_5 = \frac{1}{2},
	\end{multline}
	and
	\begin{multline}
		\PP\left[S_{j+1}\geq (S_{j}+S_{j+2})/2 \right] \\ = 5!\int_{0 \leq t_1 \dots \leq t_5 \leq 1} \mathbbm{1}\{t_4 \geq (t_3 + t_5)/2\}dt_1 \dots dt_5 \\ 
		= 5!\int_{0 \leq t_3 \dots \leq t_5 \leq 1} \frac{t_3^2}{2}  \mathbbm{1}\{t_4 \geq (t_3 + t_5)/2\} dt_3 dt_4 dt_5 \\
	\qquad 	= 5!\int_{0 \leq t_4 \leq t_5 \leq 1} \frac{(2t_4 - t_5)^3}{6} \mathbbm{1}\{2t_4 - t_5 \geq 0\}dt_4 dt_5 \\
		= 5!\int_{0}^1 \frac{t_5^4}{48} dt_5 = \frac{1}{2}.
	\end{multline}
	This proves \eqref{d1-lemma}. 

	Next, note that from \eqref{d1-lemma}, we have
	\begin{multline}
	\EE\left[\mathbbm {1}\{(S_{j-2}+S_{j})/2\leq S_{j-1} \} \mathbbm {1} \{S_{j+1}\leq (S_{j}+S_{j+2})/2 \}\right] \\
	= \EE\Big[\mathbbm {1}\{(S_{j-2}+S_{j})/2\leq S_{j-1} \}  \times \left\{1 -  \mathbbm {1} \{S_{j+1} > (S_{j}+S_{j+2})/2 \}   \right\}\Big] \\
	= \EE\left[\mathbbm {1}\{(S_{j-2}+S_{j})/2\leq S_{j-1} \}\right] \\ - \EE\left[\mathbbm {1}\{(S_{j-2}+S_{j})/2\leq S_{j-1} \} \mathbbm {1} \{S_{j+1} > (S_{j}+S_{j+2})/2 \}\right] \\
	= \frac{1}{2} - \EE\left[\mathbbm {1}\{(S_{j-2}+S_{j})/2\leq S_{j-1} \} \mathbbm {1} \{S_{j+1} > (S_{j}+S_{j+2})/2 \}\right].
	\end{multline}

	
	Then, by  direct calculations, we have
	\begin{multline}
		\EE\left[\mathbbm {1}\{(S_{j-2}+S_{j})/2\leq S_{j-1} \} \mathbbm {1} \{S_{j+1} > (S_{j}+S_{j+2})/2 \}\right] \\ = 5! \int_{0\leq t_1\leq \dots \leq t_5\leq 1} \mathbbm{1}\left\{ 2t_2 \geq  t_3 + t_1 \right\} \mathbbm{1}\left\{ 2t_4 >  t_3 + t_5 \right\} \\ {\rm d}t_1 \dots {\rm d}t_5\\
	\qquad \qquad 	= 5! \int_{0\leq t_2\leq \dots \leq t_5\leq 1} (2t_2 -t_3)\mathbbm{1}\left\{2 t_2 \geq t_3  \right\} \\ \times \mathbbm{1}\left\{ 2t_4 >  t_3 + t_5 \right\} {\rm d}t_2\dots {\rm d}t_5\\
		= 5! \int_{0\leq t_3\leq \dots \leq t_5\leq 1} \frac{t_3^2}{4}\mathbbm{1}\left\{ 2t_4 >  t_3 + t_5 \right\} {\rm d}t_3\dots {\rm d}t_5\\
	\qquad 	= 5! \int_{0\leq t_4\leq  t_5\leq 1} \frac{\left(2t_4-t_5\right)^3}{4\times 3}\mathbbm{1}\left\{ 2t_4 >  t_5 \right\}{\rm d}t_4 {\rm d}t_5\\
		= 5! \int_{0\leq  t_5\leq 1} \frac{t_5^4}{4\times 3\times 4 \times 2}{\rm d}t_5 
		%= \frac{5!}{4 \times 3\times 4 \times 2 \times 5}
		= \frac{1}{4},
	\end{multline}
which implies \eqref{d3-lemma}.
	
	Finally, note that 
	\begin{multline}
		\frac{1}{2} = \EE\left[\mathbbm {1}\left\{2 S_{j-1}\geq S_{j} + S_{j-2} \right\}\right] \\= \EE\left[\mathbbm {1}\left\{2 S_{j-1}\geq S_{j} + S_{j-2} \right\}\mathbbm {1}\left\{2 S_{j+1}\geq S_{j} + S_{j+2} \right\}\right] \\ + \EE\left[\mathbbm {1}\left\{2 S_{j-1}\geq S_{j} + S_{j-2} \right\}\mathbbm {1}\left\{2 S_{j+1}\leq S_{j} + S_{j+2} \right\}\right],
	\end{multline}
	which implies \eqref{treez}. 
	
	
	For the general case $n\geq 5$ and $3\leq j \leq n-2$, let us first note that the conditional joint distribution of $(S_{j-2},S_{j-1},S_j, S_{j+1},S_{j+2})$ given all the other order statistics is that of an order statistics from an independent  sample of size 5 from the uniform distribution on $[S_{j-3}, S_{j+3}]$, with $S_0=0$ and $S_{n+1}=1$. See, for example, Theorems 2.4.1 to  2.4.4 of \cite{arnold}.
	Finally, note that all the sets involved in \eqref{d1-lemma} and \eqref{d3-lemma} are invariant to rescaling and translation, making all the calculations above for the uniform distribution $[0,1]$ valid for the uniform distribution on $[S_{j-3}, S_{j+3}]$. This completes the proof. 
	
	
	\medskip
	
	b)  If $n=3$ and $j=1$ or $j^\prime = n$, 
	 in the case $[a,b]=[0,1]$, we can write 
	\begin{multline} \label{reety}
		\PP\left[S_{j+1} \leq (S_{j}+S_{j+2})/2  \right]  
		 =3! \int _{ 0\leq t_1\leq t_2\leq t_3\leq 1}\mathbbm{1}\left\{ 2t_2 \leq t_1 + t_3 \right\}{\rm d}t_1{\rm d}t_2{\rm d}t_3\\
	=	\PP\left[ (S_{j^\prime -2}+S_{j^\prime })/2 \leq S_{j^\prime -1}   \right] = \frac{1}{2}  .
	\end{multline}
	When $n=4$ and $j=2$ (resp. $j^\prime = n-1$), it suffices to consider the conditional distribution of $(S_j,S_{j+1},S_{j+2})$ given $S_1$ (resp. $(S_{j^\prime },S_{j^\prime +1},S_{j^\prime +2})$ given $S_n$), which is uniform. By arguments already used above, the  calculation \eqref{reety} is valid in this case too. Now the proof is complete. \end{proof}

\medskip

Let us recall few elementary properties of the order statistics for uniform distribution.
Let $U_{1},\ldots,U_{n}$ be the \emph{order statistics} of an independent uniform sample on $[0,1]$. Let $U_{0}=0$ and $U_{n+1}=1$. Then, for any $0\leq l < k \leq n+1$, the variables $U_{k} - U_{l}$ and $U_{k-l} $ have the same distribution, that is a beta distribution ${\rm Beta} (k-l,n-(k-l)+1)$. On the other hand, for any $\alpha >0$, we have 
\begin{multline}\label{beta_mom}
	\mathbb{E}\left[ U_{r} ^\alpha  \right] = \frac{ B(\alpha+r,n-r+1)}{B(r,n-r+1)} = \frac{\Gamma (\alpha+r) }{\Gamma (r)} \frac{\Gamma (n+1) }{\Gamma (n+\alpha +1)}, \\ \qquad \text{with} \quad r=k-l,
\end{multline}
where $B(\cdot,\cdot)$ denotes the beta function and $\Gamma(\cdot)$ the gamma function.
It also worthwhile to notice that $U_{k} - U_{l}$ and $U_{l}$ are independent, and the same is true for $U_{k} - U_{l}$ and $U_{k}$. Finally, note that 
\begin{equation}\label{beta_mom2}
	x^{s}\left( \frac{1}{1+s/x} \right)^{1-s}\leq  \frac{\Gamma (x+s) }{\Gamma (x)} \leq x^s,  \qquad \text{with} \quad \forall x\geq 1, 0\leq s\leq 1.
\end{equation}
See \cite{wendel}. Repeated application of this double inequality yields
\begin{equation}\label{beta_mom3}
	\mathbb{E}\left[ U_{r} ^\alpha  \right] \leq C(n,\alpha)\left(\frac{r}{n+1}\right)^{\alpha}, \qquad  r=k-l,
\end{equation}
with $C(n,\alpha)= \left\{(n+\alpha+1)/(n+1)\right\}^{1-\alpha}$ a bounded quantity. See also \cite{golo1}.


\medskip


\begin{lemma}\label{d1d2-lem_b}
	Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of a sample of independent uniform $[0,1]$ variables.
	a)	Let $3\leq j \leq n-2$. Then
	\begin{equation}\label{cross_2}
		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1}\{2S_{j+1} < S_j + S_{j+2} \} \right]	= \frac{3}{4(n+1)}
	\end{equation}
	and
	\begin{equation}\label{cross_2}
		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1}\{2S_{j-1} > S_{j-2} + S_j \} \right]	
		= 	\frac{1}{(n+1)}.
	\end{equation}
	
	
	b) For $j\in\{1,2,n-1,n\}$, we have 
	\begin{multline}\label{ext_1a}
		\EE[  \{ S_1 +S_2\}\mathbbm{1}\{2S_2 \leq S_1 +S_3 \}] \\ =
		\EE[  \{ 2- (S_{n-1} +S_n)\}\mathbbm{1}\{2S_{n-1} \geq S_{n} +S_{n-1} \}] = \frac{5}{4(n+1)},
	\end{multline}
	and
	\begin{multline}\label{ext_1b}
		\EE\left[ \{ S_3 -  S_1\}\mathbbm{1}\{2S_3 \leq S_2 +S_4 \} \right ] = \frac{3}{4(n+1)}
	\\	=\EE\left[ \{ S_n -  S_{n-2}\}\mathbbm{1}\{2S_{n-2} \geq S_{n-3} +S_{n-1} \} \right ].
	\end{multline}
\end{lemma}

\medskip


\begin{proof}[Proof of Lemma \ref{d1d2-lem_b}]
	\emph{a)}  First, consider $n=5$ and $j=3$. In this case, by direct calculations, we have
	\begin{multline}
		\EE\left[\left(S_{j+1} - S_{j-1}\right)\mathbbm{1}\{2S_{j+1} > S_j + S_{j+2} \} \right] \\
		= 5!\int_{0\leq t_1\leq\dots\leq t_5 \leq 1} (t_4 - t_2) \mathbbm{1}\{2t_4 - t_5 > t_3\} {\rm d}t_1\dots{\rm d}t_5\\
		= 5!\int_{0\leq t_2\leq\dots\leq t_5 \leq 1}\{t_2 t_4 - t_2^2\} \mathbbm{1}\{2t_4 - t_5 > t_3\}  {\rm d}t_2\dots{\rm d}t_5\\
		=5!\int_{0\leq t_3\leq\dots\leq t_5 \leq 1} \left(\frac{t_3^2t_4}{2} - \frac{t_3^3}{3}\right) \mathbbm{1}\{2t_4 - t_5 > t_3\} \\ {\rm d}t_3\dots{\rm d}t_5\\
		=5!\int_{0\leq t_3\leq\dots\leq t_5 \leq 1} \int_{0}^{2t_4 - t_5}\left(\frac{t_3^2t_4}{2} - \frac{t_3^3}{3}\right) \mathbbm{1}\{2t_4 - t_5 > 0\} \\ {\rm d}t_3\dots{\rm d}t_5\\
		= 5! \int_{0 \leq t_4\leq t_5 \leq 1} \left\{ \frac{ (2t_4 - t_5)^3 t_4}{6} - \frac{  (2t_4 - t_5)^4}{ 12}\right\} \\ \times \mathbbm{1}\{2t_4 - t_5 > 0\}  {\rm d}t_4{\rm d}t_5\\
		= 5! \int_{0 \leq t_4\leq t_5 \leq 1}    \frac{ t_5(2t_4 - t_5)^3}{12}   \mathbbm{1}\{2t_4 - t_5 > 0\}  {\rm d}t_4{\rm d}t_5\\
		= 5!\int_0^1 \left\{  \frac{t_5^5}{ 12\times 4\times 2} \right\} {\rm d}t_5= \frac{5}{24}.
	\end{multline}
	In addition, applying \eqref{beta_mom} with $n=5$, $r=2$ and $\alpha=1$, we have 
	$\EE\left[S_{j+1} - S_{j-1} \right] = 1/3$,
	and thus, in the case $n=5$ and $j=3$, we have
	\begin{equation}
		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1} \{2S_{j+1} <  S_j + S_{j+2} \} \right]= \frac{1}{8}.
	\end{equation}
	Let us note that in the case of a sample of size 5 from a uniform distribution on some interval $[a,b]$, we get 
	\begin{equation}\label{zoom}
		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1} \{2S_{j+1} <  S_j + S_{j+2} \} \right]= \frac{b-a}{8}.
	\end{equation}	
This is because if $U_{1},\ldots, U_5$ is the order statistics of an independent uniform sample on $[0,1]$, then $S_j = a+ (b-a)U_j$, $1\leq j\leq 5$, is the order statistics from  an independent uniform sample on $[a,b]$. Moreover, we have
	\begin{multline}
		(b-a)	\EE\left[\left(U_{j+1} - U_{j-1}\right) \mathbbm{1} \{2U_{j+1} <  U_j + U_{j+2} \} \right] \\ = \EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1} \{2S_{j+1} <  S_j + S_{j+2} \} \right].
	\end{multline}	
	For the general case $n\geq 5$ and $3\leq j \leq n-2$, using again Theorems 2.4.1 to  2.4.4 of \cite{arnold}, the fact that the density of the uniform on $[S_{j+3}, S_{j-3}]$ is $1/(S_{j+3} - S_{j-3} )$, and \eqref{zoom}, we can write
	\begin{multline}
		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1} \{2S_{j+1} <  S_j + S_{j+2} \} \right] \\
		= \EE \left\{ \EE \left[ \left(S_{j+1} - S_{j-1}\right) \mathbbm{1} \{2S_{j+1} <  S_j + S_{j+2} \} \mid S_{j-3},S_{j+3}\right]\right\}\\
		= \EE\left[S_{j+3} - S_{j-3} \right] \times \frac{1}{8} = \frac{3}{4(n+1)},
	\end{multline}
	where for the last equality we use \eqref{beta_mom} with $l=n-3$,  $k=n+3$  and $\alpha=1$.
	
	For the second identity, we start again with the case $n=5$ and $j=3$, and we get 
	%	\begin{multline}\label{zoom2}
		%		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1}\{2S_{j-1} > S_j + S_{j-2} \} \right]\\
		%		= 5! \int_{0\leq t_1 \leq \dots \leq t_5 \leq 1} (t_4 - t_2)\mathbbm{1}\left\{ 2t_2-t_1 \geq t_3\right\}{\rm d}t_1\dots {\rm d}t_5\\
		%		= 5! \int_{0\leq t_1 \leq \dots \leq t_4 \leq 1} (t_4 - t_2)(1-t_4)\mathbbm{1}\left\{ 2t_2-t_1 \geq t_3\right\}{\rm d}t_1\dots {\rm d}t_4\\
		%		= 5! \int_{0\leq t_2 \leq t_3 \leq t_4 \leq 1} (t_4 - t_2)(1-t_4)(2t_2-t_3)\mathbbm{1}\left\{ 2t_2-t_3 \geq 0\right\}{\rm d}t_2{\rm d}t_3 {\rm d}t_4\\
		%		= 5! \int_{0\leq t_2  \leq t_4 \leq 1} (t_4 - t_2)(1-t_4)\frac{t_2^2}{2}{\rm d}t_2 {\rm d}t_4\\
		%		= \frac{5!}{2} \int_{0\leq t_2  \leq t_4 \leq 1}\left\{-t_4^2t_2^2 + t_4t_2^2+ t_4t_2^3- t_2^3 \right\}{\rm d}t_2 {\rm d}t_4\\
		%		=\frac{5!}{2} \int_0^1\left\{-\frac{t_4^5}{3} +\frac{t_4^4}{3} +\frac{t_4^5}{4} - \frac{t_4^4}{4}\right\} {\rm d}t_4 = \frac{5!}{ 12\times 5\times 6 \times 2}= \frac{1}{6}.
		%	\end{multline}
	
	\begin{multline}\label{zoom2}
		\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1}\{2S_{j-1} > S_j + S_{j-2} \} \right]\\
		= 5! \int_{0\leq t_1 \leq \dots \leq t_5 \leq 1} (t_4 - t_2)\mathbbm{1}\left\{ 2t_2-t_1 \geq t_3\right\}{\rm d}t_1\dots {\rm d}t_5\\
		= 5! \int_{0\leq t_2 \leq \dots \leq t_5 \leq 1} (t_4 - t_2)(2t_2-t_3)\mathbbm{1}\left\{ 2t_2 \geq t_3\right\}{\rm d}t_2\dots {\rm d}t_4\\
		=5!\int_{0\leq t_3\leq t_4  \leq t_5 \leq 1}  \frac{t_4t_3^2}{2\times 2} - \frac{t_3^3}{2\times 2\times 3} -\frac{t_3^3}{ 2\times 2\times 2}{\rm d}t_3{\rm d}t_4{\rm d}t_5\\
		= 5! \int_{0\leq t_4  \leq t_5 \leq 1}  \left\{\frac{t_4^4}{2\times 2\times 3}-\frac{t_4^4}{2\times 2\times 3\times 4}-\frac{t_4^4}{2^5} \right\}  {\rm d}t_4{\rm d}t_5\\
		=5! \int_0^1\frac{t_5^5}{5\times 4\times 8}{\rm d}t_5 = \frac{5!}{ 5\times 4\times 8\times 6 }= \frac{1}{8}.
	\end{multline}
	Therefore, by the same arguments as above, for the general case $n\geq 5$ and $3\leq j \leq n-2$, we get
	\begin{equation}
		\EE\left[\{S_{j+1} - S_{j-1}\}\mathbbm{1}\{2S_{j-1} >  S_j + S_{j-2} \}  \right]  =\EE\left[S_{j+3}- S_{j-3}\right]\times \frac{1}{8} =\frac{3}{4(n+1)}.
	\end{equation}
	
	\medskip
	
	\emph{b)} For $j=1$, we can use the fact that the conditional distribution of the order statistics $S_1,S_2,S_3$, given all the other order statistics in the uniform $[0,1]$ sample of $[0,1]$, only depends on $S_4$. Moreover, this conditional distribution is uniform on $[0,S_4]$. Then, using \eqref{zoom}, we get  the following conditional expectation expression
	\begin{multline}\label{zoom3}
		\EE[  \{ S_1 +S_2\}\mathbbm{1}\{2S_2 \leq S_1 +S_3 \}\mid S_4] \\ =S_4 \times 3!  \times \left(\frac{1}{8}-\int_{0\leq t_1 \leq t_2 \leq t_3 \leq 1} (t_1+t_2)\mathbbm{1}\{2t_2\geq t_1+t_3\}{\rm d}t_1 {\rm d}t_2{\rm d}t_3\right)\\
		= S_4 \times 3! \left(\frac{1}{8}-\frac{7}{2\times 3  \times 2^{4}}\right) =   \frac{5S_4}{16}.
	\end{multline}
	Integrating with respect to $S_4$, and using \eqref{beta_mom} we get the first part of \eqref{ext_1a}.
	For the second one, i.e., when $j=n$, we note that the distributions of $(1-S_n,\ldots, 1-S_1)$ and $(S_1,\ldots ,S_n)$ coincides. The result then follows from this symmetry property  and the first part of \eqref{ext_1a}.
	
	For $j= 2$, by similar arguments for the conditional distribution and direct calculations, we get
	\begin{multline}\label{zoom4}
		\!\!	\EE\left[ \{ S_3 \!- \! S_1\}\mathbbm{1}\{2S_3 \leq S_2 +S_4 \}\mid S_5\right ] \\=S_5 \times 4! \int _{ 0\leq t_1 \leq \dots \leq t_4 \leq 1} \!(t_3 -t_1 )\mathbbm{1}\{2t_3 \leq t_2 +t_4 \} {\rm d}t_1\!\dots \!{\rm d}t_4\\
		= S_5 \times 4! \Big( \frac{1}{3\times 4\times 5} -\int _{ 0\leq t_1 \leq \dots \leq t_4 \leq 1} (t_3 -t_1 )\mathbbm{1}\{2t_3 \geq t_2 +t_4 \} {\rm d}t_1\dots {\rm d}t_4 \Big)  = \frac{3S_5}{20}.
	\end{multline} 
	Integrating with respect to $S_5$, we get the first equality of \eqref{ext_1b}. The second part of \eqref{ext_1b} follows by the symmetry property of the uniform distribution,  as we already used for  \eqref{ext_1a}. \end{proof}



\medskip



\begin{lemma}\label{d-lemma}
	Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of a sample of independent uniform $[0,1]$ variables. 	Let $\varphi$ be an $s-$Hölder continuous function with $s\in(0,1]$ and the Hölder  constant $L_\varphi$. 
	Then
	\begin{equation}
		\EE\left[\widehat d_j^2 \varphi(S_j) \right] = L_\varphi O(n^{-s}) +  
		\left\{ 
		\begin{tabular}{lll}
			$\dfrac{3}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{3,\ldots, n-2 \}$,\\
			\\ 	$\dfrac{5}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{2, n-1\}$,\\
			\\
			$\dfrac{1}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{1,  n \}$.
		\end{tabular} 
		\right. 
	\end{equation}
\end{lemma}

\medskip

\begin{proof}[Proof of Lemma \ref{d-lemma}]  Recall that $\lesssim$ means that the left side is bounded by a positive constant times the right side.  
	Let us first note that, in the case $3\leq j \leq n-2$, by Lemma \ref{d1d2-lem} and direct calculations using the explicit representation \eqref{dm_explicit} of the $\widehat d_j$,
	$$
	\EE\left[\widehat d_j^2 \mid  S_{j-3}, S_{j+3} \right]=\EE\left[\widehat d_j^2   \right]= \frac{3}{2}.
	$$
	This is a consequence of the fact that $(S_{j-2},S_{j-1},S_j, S_{j+1},S_{j+2})$ given all the other order statistics is that of an order statistic from an independent  sample of size 5 from the uniform distribution on $[S_{j-3}, S_{j+3}]$, with $S_0=0$ and $S_{n+1}=1$.
	
	
	Next, we write
	\begin{multline}
		\EE\left[\widehat d_j^2 \varphi(S_j) \right] = \EE\left[\varphi(S_{j-3})\EE\left[\widehat d_j^2 \mid  S_{j-3}, S_{j+3} \right] \right] \\ + \EE\left[\widehat  d_j^2 \left\{\varphi(S_j) - \varphi(S_{j-3}) \right\} \right] \\
		= \frac{3}{2} \EE\left[\varphi(S_{j-3}) \right] + \EE\left[\widehat  d_j^2 \left\{\varphi(S_j) - \varphi(S_{j-3}) \right\} \right].
	\end{multline}
	By the Hölder continuity of $\varphi$ and the fact that $\widehat d_j\in\{0,1,2\}$, using \eqref{beta_mom3}, we have 	
	\begin{equation*}
	\left| \EE\left[\widehat  d_j^2 \left\{\varphi(S_j) - \varphi(S_{j-3}) \right\} \right] \right|\leq 
	4L_{\varphi}\EE\left[|S_j - S_{j-3} |^s\right] \lesssim \frac{L_\varphi }{(n+1)^{s}}.
	\end{equation*}
	On the other hand, 
	$$
	\left| \EE\left[\varphi(S_{j-3}) \right] - \EE\left[\varphi(S_{j}) \right]\right|\lesssim \frac{L_\varphi }{(n+1)^{s}}.
	$$		
	Gathering facts, 
	\begin{equation*}
	\left|\EE\left[\widehat d_j^2 \varphi(S_j) \right]  -\frac{3}{2} \EE\left[\varphi(S_{j}) \right] \right| \lesssim \frac{L_\varphi }{(n+1)^{s}},  \qquad 3\leq j \leq n-2.
	\end{equation*}
	
	
	In the case $j=1$, by \eqref{dm_explicit_end_l} we have $\widehat d_1^2= \widehat d_1$
	and thus
	\begin{equation}
		\EE\left[\widehat d_1^2\varphi(S_1 )\right] =\EE\left[\widehat d_1 \varphi(S_1)\right]  = \EE\left[\EE\left[\widehat d_1\mid S_4\right] \varphi(S_4)\right] +\EE\left[\widehat d_1 \{\varphi(S_1)-\varphi(S_4)\}\right]. 
	\end{equation}
	Then, using \eqref{treez} and the Hölder continuity of $\varphi$, we get
	\begin{equation}
		\left|\EE[d_1^2\varphi(S_1 )] - \frac{1}{2} \EE[\varphi(S_1)]\right| \lesssim \frac{L_\varphi }{(n+1)^{s}}. 
	\end{equation}
	By symmetry, we get the same approximation error with $j=n$.
	
	In the case $j=2$, by \eqref{dm_explicit_end_r}, we have 
	$
	\widehat	d_2 = 1 + \mathbbm {1}\{ 2S_3 \leq S_2 + S_4\},
	$
	and expanding the squares we get
	\begin{equation}
		\EE\left[\widehat d_2^2 \mid  S_1, S_5 \right] = 1 + 3\EE\left[\mathbbm{1}\{2S_3 \leq S_2 + S_4 \} \mid S_1, S_5  \right].
	\end{equation}
	Repeating arguments used above and by another direct calculation %on the complement 
	yields
	\begin{equation}
		\EE[\mathbbm {1}\{ 2S_3 \leq S_2 + S_4\}\mid S_1, S_5]  = 3 ! \int _{ 0\leq t_2\leq t_3\leq t_4\leq 1}\mathbbm{1}\left\{ 2t_3 \leq t_2 + t_4 \right\}{\rm d}t_2{\rm d}t_3{\rm d}t_4  =  \frac{1}{2}.
	\end{equation}
	Thus 
	\begin{equation}
		\left|	\EE \left[\widehat d_2^2\varphi(S_2 )\right]- \frac{5}{2}\EE[\varphi(S_2 )]\right| \lesssim \frac{L_\varphi }{(n+1)^{s}}.
	\end{equation}
	By symmetry, we get the same approximation error with $j=n-1$. The proof is now complete. 	
\end{proof}

\medskip

For the following calculations, it is also useful to consider a proxy of $\widehat c_j$ as proposed by \cite{leluc2024speeding}. For simplicity, we introduce this proxy directly in the case of a general, not necessarily uniform density $f_T$.  More precisely, for $ 2\leq j \leq n-1$, let 
\begin{equation}\label{def_ctilde}
	\widetilde c_j = n V_j (\mathfrak S) = n\left[F_T\left(\frac{S_{j}+S_{j+1}}{2}  \right) - F_T\left(\frac{S_{j-1}+S_{j}}{2}  \right) \right],
\end{equation}
and 
$$
\widetilde c_1 =n F_T\left(\frac{S_{1}+S_{2}}{2}  \right),\quad \widetilde c_{n} =n \left[1-F_T\left(\frac{S_{n-1}+S_{n}}{2}  \right)\right],
$$
and note that for $ 3\leq j \leq n-2$
\begin{multline}
	\left| \widetilde c_j - \widehat c_j \right|\leq
	2\left[F_T\left(\frac{S_{j}+S_{j+1}}{2}  \right) - F_T\left(\frac{S_{j-1}+S_{j}}{2}  \right) \right]\\+ \left[F_T\left(\frac{S_{j}+S_{j+2}}{2}  \right) - F_T\left(\frac{S_{j-2}+S_{j}}{2}  \right) \right]
	\\\leq  \|f_T\|_\infty
	\left[  S_{j+1} - S_{j-1} + \frac{S_{j+2} - S_{j-2}}{2} \right] .
\end{multline}
Moreover,
\begin{equation*}
\left| \widetilde c_1 - \widehat c_1 \right|\leq \|f_T\|_\infty  
\left[ S_{1}+S_{2} +  \frac{S_{1}+S_{3}}{2} \right]  , \qquad 
\left|\widetilde c_2 - \widehat c_2 \right|\leq \|f_T\|_\infty
\left[  S_{3} - S_{1} + \frac{S_{2}+S_{4}}{2} \right],  
\end{equation*}
and
$$
\left| \widetilde c_{n-1} - \widehat c_{n-1} \right|\leq \|f_T\|_\infty  
\left[ S_{n}-S_{n-2} + 1-  \frac{S_{n-3}+S_{n-1}}{2} \right]  , 
$$
$$ 
\left|\widetilde c_n - \widehat c_n \right|\leq \|f_T\|_\infty
\left[ 3-  S_{n-1} - S_{n}-  \frac{S_{n-2}+S_{n}}{2} \right].
$$
Gathering facts, we deduce that for any $k\geq 1$, a constant $C_k$  exists such that 
\begin{equation}\label{subst}
	\left|	\EE	\left( \widetilde c^k_j \right) - \EE	\left( \widehat c^k_j \right)  \right|  \leq C_k n^{-1}, \qquad 1 \leq j\leq n. 
\end{equation}
Moreover,  by \eqref{beta_mom3}, it is easy to check that, for any $k\geq 1$, a constant $C^\prime _k$  exists such that 
\begin{equation}\label{subst2}
	\EE	\left( \widetilde c^k_j \right)    \leq C^\prime _k , \qquad 1 \leq j\leq n. 
\end{equation}


\medskip


We are now ready for the next moment calculations, in the uniform case. 

\medskip

\begin{lemma}\label{lem_mom_c}
	Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of a sample of independent uniform $[0,1]$ variables. 		Let $\varphi$ be $s-$Hölder continuous with Hölder constant $L_\varphi$. 
	Then,  
	\begin{equation*}
		\EE\left[\widehat c_j^2 \varphi(S_j) \right] =  O(n^{-s})  +  
		\left\{ 
		\begin{tabular}{lll}
			$\dfrac{3}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{2,\ldots, n-1 \},$\\
			\\ 	$\dfrac{7}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{1,  n \},$\\
		\end{tabular} 
		\right. 
	\end{equation*}
	with the constant in $ O(n^{-s})$   depending only on $s$, $L_\varphi$ and $ \|f_T\|_\infty	$ (in the current case $ \|f_T\|_\infty=1	$).
\end{lemma}

\medskip

\begin{proof}[Proof of Lemma \ref{lem_mom_c}]
	First of all, let us point out that because of \eqref{subst} it suffices to derive the result with 
	$\widehat c_j$ replaced by $\widetilde c_j$.
	When $3\leq j \leq n-2$, using  \eqref{def_ctilde} in the uniform case,  \eqref{beta_mom} with $n=5$, $r=2$ and $\alpha = 2$, and the Markov property recalled after \eqref{beta_mom}, we get 
	\begin{multline}
		\EE \left[\widetilde c_j^2 \mid S_{j-3},S_{j+3}\right]=  \frac{n^2}{4}\EE \left[(S_{j+1} - S_{j-1})^2\mid S_{j+3}, S_{j-3}\right]\\
		= \frac{n^2}{4}(S_{j+3}- S_{j-3})^2 \times \frac{\Gamma (4)}{\Gamma (2)} \times \frac{\Gamma (6)}{\Gamma (8)}.
	\end{multline}
	On the other hand, applying again \eqref{beta_mom} with $n\geq 5 $ and $\alpha = 2$, we get
	\begin{multline}
		\EE \left[\widetilde c_j^2 \varphi(S_j) \right] = \EE \left\{\varphi(S_{j-3})\EE \left[\widetilde c_j^2  \mid S_{j-3},S_{j+3} \right]\right\} \\ + \EE \left[\widetilde c_j^2 \{\varphi(S_j)- \varphi(S_{j-3})\} \right] \\
		%=	\EE \left[\widetilde c_j^2 \mid S_{j-3},S_{j+3}\right] \\
		=  \frac{n^2}{4}\EE \left[(S_{j+3}- S_{j-3})^2 \right]\times \frac{\Gamma (4)}{\Gamma (2)} \times \frac{\Gamma (6)}{\Gamma (8)} \times  \EE\left[  \varphi(S_{j-3}) \right] \\ + \EE \left[\widetilde c_j^2 \{\varphi(S_j)- \varphi(S_{j-3})\} \right]
		\\	= \frac{3}{2} \times \frac{n^2}{(n+1)(n+2)}\times  \left[\EE\left[  \varphi(S_{j}) \right]  +    \left\{\EE\left[  \varphi(S_{j-3}) \right]-  \EE\left[  \varphi(S_{j}) \right] \right\}\right]\\ + \EE \left[\widetilde c_j^2 \{\varphi(S_j)- \varphi(S_{j-3})\} \right].
	\end{multline}
	Based on arguments already used in the previous proofs, after some straightforward but quite lengthy calculations, we get
	$$
	\left| 	\EE \left[\widetilde c_j^2 \varphi(S_j) \right] - \frac{3}{2} \EE\left[  \varphi(S_{j}) \right] \right| \leq \frac{C}{(n+1)^{s}},
	$$
	with some constant $C$ depending only on $s$, $L_\varphi$ and $\|f_T\|_\infty$  (in the current case $ \|f_T\|_\infty=1	$). 
	
	We now consider the extreme case $j=1$. 
	First, direct calculation yields
	\begin{multline}
		\EE[\widetilde c_1^2 \mid  S_3]=  \frac{n^2}{4}\EE[(S_1+S_2)^2 \mid  S_3]
		\\ =\frac{(nS_3)^2}{2}  \int _{0\leq t_1 \leq t_2 \leq 1} (t_1 + t_2)^2 {\rm d}t_1 {\rm d}t_2\\
		=\frac{1}{2} (nS_3)^2\times \frac{7}{3}\int _{0}^1  t_2^3  {\rm d}t_2 = \frac{7}{24}n^2S_3 ^2,
	\end{multline}	
	and 
	\begin{equation}\label{tyze}
		\EE[\widetilde c_1^2  ]= 	\EE\left[\frac{7}{24}n^2S_3 ^2\right]= \frac{7}{2} + O(n^{-1}).
	\end{equation}
	On the other hand, using the Hölder continuity, Cauchy-Schwarz inequality and the bound \eqref{subst}, we get	
	\begin{equation}
		\left|\EE\left[\widetilde c_1^2 \varphi(S_1)\right]- \varphi(0)\EE\left[  \widetilde c_1^2  \right]\right|\lesssim  \frac{L_\varphi}{(n+1)^{s}} ,
	\end{equation}
	and therefore, again using the  Hölder continuity and \eqref{tyze},
	\begin{equation}
		\left|\EE\left[\widetilde c_1^2 \varphi(S_1)\right]- \frac{7}{2}\EE[\varphi(S_1)]\right|\lesssim  \frac{L_\varphi}{(n+1)^{s}} .
	\end{equation}
	By symmetry, the same bound is valid for $\EE[\widetilde c_n^2\varphi(S_n )]$.
	
	
	Finally, let   $j=2$. Applying \eqref{beta_mom} with $n=3$, $r=2$ and $\alpha=2$, and again with $n\geq 5$, $r=2$ and $\alpha=2$, we get 
	\begin{equation}
		\EE[\widetilde c_2^2 \mid  S_4]=  \frac{n^2}{4}\EE[(S_3-S_1)^2 \mid  S_4] \\ = \frac{n^2S_4 ^2}{4} \times \frac{3}{10}, \quad \text{ and } \quad  \EE[\widetilde c_2^2 ]= \frac{3}{2} + O(n^{-1}).
	\end{equation}
	Using the Hölder continuity, Cauchy-Schwarz inequality and the bound \eqref{subst}, we also have
	\begin{equation}
		\left|\EE\left[\widetilde c_2^2 \varphi(S_2)\right]- \varphi(0)\EE\left[  \widetilde c_2^2  \right] \right|\lesssim  \frac{L_\varphi}{(n+1)^{s}} ,
	\end{equation}
	and therefore again using the  Hölder continuity, 
	\begin{equation}
		\left|\EE\left[\widetilde c_2^2 \varphi(S_2)\right]- \frac{3}{2}\EE[\varphi(S_2)] \right|\lesssim  \frac{L_\varphi}{(n+1)^{s}} ,
	\end{equation}
	By symmetry, the same bound is valid for $\EE[\widetilde c_{n-1}^2\varphi(S_{n-1} )]$.
\end{proof}




\medskip

\begin{lemma}\label{lem:cross_cd}
	Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of a sample of independent uniform $[0,1]$ variables. 		Let $\varphi$ be $s-$Hölder continuous with Hölder constant $L_\varphi$. Then,  
	\begin{equation}
		\EE\left[\widehat c_j\widehat d_j \varphi(S_j) \right]  =  O(n^{-s})+  
		\left\{ 
		\begin{tabular}{lll}
			$\dfrac{3}{4}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{2,\ldots, n-1 \},$
			\\
			\\ 	$\dfrac{11}{8}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{2,  n-1 \},$\\
			\\ 	$\dfrac{5}{8}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{1,  n \},$
		\end{tabular} 
		\right. 
	\end{equation}
	with the constant in $ O(n^{-s})$   depending only on $s$, $L_\varphi$ and $ \|f_T\|_\infty	$  (in the current case $ \|f_T\|_\infty=1	$).	
\end{lemma}

\medskip

\begin{proof}[Proof of Lemma \ref{lem:cross_cd}]
	Let $j\notin \{1,2, n-1, n\}$. By the arguments used several times in the proof of Lemma \ref{lem_mom_c}, we have  
	\begin{equation}
		\left|\EE\left[\widehat c_j \widehat d_j\varphi(S_j)\right] -  \EE\left[\varphi(S_{j-3}) \EE\left[\widehat c_j \widehat d_j | S_{j-3}, S_{j+3} \right]\right]\right|
		 \leq  \frac{C}{(n+1)^{s}},
	\end{equation}
	for some constant $C$. 
	On the other hand, using the definitions \eqref{dm_explicit} and \eqref{cm_explicit}, and the identities \eqref{zoom} and \eqref{zoom2}, 
	\begin{multline}
		\EE\left[\widetilde c_j \widehat d_j | S_{j-3}, S_{j+3}\right]  = \frac{n}{2}\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1}\{2S_{j-1} \geq S_{j-2} + S_{j}\}  \mid  S_{j-3}, S_{j+3} \right] \\ + \frac{n}{2}\EE\left[\left(S_{j+1} - S_{j-1}\right) \mathbbm{1}\{2S_{j+1} \leq S_j + S_{j+2}\}  \mid  S_{j-3}, S_{j+3} \right] 
	\\	=\frac{n}{2} \left[ \frac{1}{8} + \frac{1}{8}\right] \{S_{j+3} - S_{j-3}\}.
	\end{multline}
	Furthermore, recall that we have $\EE[S_{j+3} - S_{j-3}]=6/(n+1)$, and since $S_{j-3}$ and the increment $(S_{j+3} - S_{j-3})$ are independent, we get the statement for $j\notin \{1,2, n-1, n\}$.
	
	It remains to study the extreme  cases, and for this purpose we replace $\widehat c_j$ by $\widetilde c_j$. For $j= 2$, by the definitions and the Hölder continuity, we have  
	\begin{multline}
		\EE[\widetilde c_2 \widehat d_2\varphi(S_2)  ]=  \frac{n}{2}\EE[ \{ S_3 -S_1\}\varphi(S_2)] \\ +\frac{n}{2}\EE[ \{ S_3 -S_1\}\mathbbm{1}\{2S_3 \leq S_2 +S_4 \}\varphi(S_2)]\\ = \varphi(0)\frac{n}{2}\EE[  (S_3 -S_1)] \\ +\varphi(0) \frac{n}{2}\EE[ \{ S_3 -S_1\}\mathbbm{1}\{2S_3 \leq S_2 +S_4 \} ] +  O(n^{-s})	.
	\end{multline}
	On the other hand, by \eqref{ext_1b} we have 
	\begin{equation}
		\EE\left[ \{ S_3 -S_1\}\mathbbm{1}\{2S_3 \leq S_2 +S_4 \} \right ]=  \frac{3}{4(n+1)}.
	\end{equation} 
	and therefore 
	\begin{equation}
		\left|\EE[\widetilde c_2 \widehat d_2\varphi(S_2)  ] - \frac{11}{8}\EE[\varphi(S_2)]\right|\leq 
		O(n^{-s}) .
	\end{equation}
	By symmetry, a similar result is valid for $j= n-1$.
	
	For $j=1$ we only have 
	\begin{equation}
		\EE[\widetilde c_1 \widehat d_1\varphi(S_1)  ]= \frac{n}{2}\EE[ \{ S_1 +S_2\}\mathbbm{1}\{2S_2 \leq S_1 +S_3 \}\varphi(S_1)].
	\end{equation}
	By \eqref{ext_1a}, 
	\begin{equation}
		\EE[  \{ S_1 +S_2\}\mathbbm{1}\{2S_2 \leq S_1 +S_3 \} ] =   \frac{5}{4(n+1)},
	\end{equation}
	and thus 
	\begin{equation}
		\EE[\widetilde c_1 \widehat d_1\varphi(S_1)  ]= \frac{5}{8}\EE[\varphi(S_1)]  + O(n^{-s}).
	\end{equation} 
	The same result is valid for $j= n$. From this, we deduce the statement in the case $j\in\{1,n\}$ and thus the proof is complete. \end{proof}

\medskip


\begin{corollary}\label{variance_bound}
	Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of a sample of independent uniform $[0,1]$ variables. 		Let $\varphi$ be $s-$Hölder continuous with Hölder constant $L_\varphi$. Then, 
	\begin{equation}
		\EE\left[\{ \widehat c_j -\widehat d_j\}^2\varphi(S_j)\right]  =  O(n^{-s})+  
		\left\{ 
		\begin{tabular}{lll}
			$\dfrac{3}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{3,\ldots, n-2 \},$\\
			\\ 	$\dfrac{5}{4}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{2, n-1\},$\\
			\\ $\dfrac{11}{4}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{1,  n \},$
		\end{tabular} 
		\right. 
	\end{equation}
	with the constant in $ O(n^{-s})$   depending only on $s$, $L_\varphi$ and $ \|f_T\|_\infty	$  (in the current case $ \|f_T\|_\infty=1	$).	
\end{corollary}

\medskip


\begin{proof}[Proof of Corollary \ref{variance_bound}]
	We have
	\begin{equation}
		\EE\left[\{ \widehat c_j -\widehat d_j\}^2\varphi(S_j)\right] = \EE\left[\widehat c_j ^2\varphi(S_j)\right]
		+ \EE\left[\widehat d_j^2\varphi(S_j)\right] - 2\EE\left[\widehat c_j \widehat d_j\varphi(S_j)\right].
	\end{equation}
	Then, the result follows by Lemmas \ref{d-lemma},  \ref{lem_mom_c} and  \ref{lem:cross_cd}. 
\end{proof}






\subsection{The moments of the weights: general case}

Below, we extend the results from the previous section to the case where $T$ admits a $\alpha_f-$Hölder continuous density $f_T$, bounded and bounded away from zero on $[0,1]$, but $f_T$ is not necessarily uniform. Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of an independent sample of $T$.

Let us first note the following fact~: for any $3\leq j \leq n-2$, and any measurable bounded function $\gamma $, with $S_0=0$ and $S_{n+1} = 1$, we have
\begin{multline}\label{trickm1}
	\EE \left[ \gamma (S_{j-2}, S_{j-1},S_j,S_{j+1}, S_{j+2}) \mid S_l, l\leq j-3, l\geq j+3 \right] \\ = \EE \left[ \gamma (S_{j-2}, S_{j-1},S_j,S_{j+1}, S_{j+2}) \mid S_{j-3} ,S_{j+3} \right].
\end{multline}
Moreover, 
\begin{multline}\label{trickm2}
	\EE \left[ \gamma (\cdot) \mid  S_{j-3} ,S_{j+3} \right]   := \EE \left[ \gamma (S_{j-2}, S_{j-1},S_j,S_{j+1}, S_{j+2}) \mid S_{j-3} ,S_{j+3} \right] \\= \frac{5!}{\{F_T(S_{j+3}) \!-\! F_T(S_{j-3})\}^5} \times \\  \int_{S_{j-3}\leq t_1 \leq \dots \leq t_5 \leq S_{j+3}} \!\gamma(t_1,\ldots,t_5) f_T(t_1)\times \cdots \times f_T(t_5) {\rm d}t_1\dots {\rm d}t_5.
\end{multline}
Next,  using the Hölder continuity assumption on $f_T$, on the one hand, we can write 
\begin{multline}
	F_T(S_{j+3}) - F_T(S_{j-3}) = f_T(S_j)\{S_{j+3} - S_{j-3} \} + R^{(1)}_{n,j}, \\  \text{ with } \quad  |R^{(1)}_{n,j}| \leq (L_f/2)\{S_{j+3} - S_{j-3} \}^{1+\alpha_f},
\end{multline}
where $L_f >0$ and $\alpha_f\in (0,1]$ are the Hölder constant and exponent of $f$, respectively. On the other hand, we have
\begin{multline}\label{trickm3}
	\int_{S_{j-3}\leq t_1 \leq \dots \leq t_5 \leq S_{j+3}} \gamma(t_1,\ldots,t_5) f_T(t_1)\times \cdots  \times f_T(t_5) {\rm d}t_1\dots {\rm d}t_5\\= f_T(S_j)^5 \int_{S_{j-3}\leq t_1 \leq \dots \leq t_5 \leq S_{j+3}} \gamma(t_1,\ldots,t_5)  {\rm d}t_1\dots {\rm d}t_5+ R^{(2)}_{n,j}
	\\  \text{ with } \quad  |R^{(2)}_{n,j}| \leq C\{S_{j+3} - S_{j-3} \}^{1+\alpha_f},
\end{multline}
with a constant $C$ depending on $L_f$, $\|f_T\|_\infty $ and $\|\gamma\|_\infty$. The identities \eqref{trickm1} and \eqref{trickm2} prove that, up to terms of order $O(n^{-\alpha_f})$, 
the value of the expectation 
$$
\EE \left[ \gamma (\cdot)  \right] = \EE\{\EE \left[ \gamma (\cdot) \mid  S_{j-3} ,S_{j+3} \right]\} ,
$$ 
does not depend on the density $f_T$. Similar arguments apply for the extreme order statistics, corresponding to $j\in\{1,2,n-1,n\}$. As a consequence, we have the following result. 

\medskip


\begin{corollary}\label{variance_bound_g}
	Let	$S_1,\ldots,S_{n}$, $n\geq 5$, be the order statistics of an independent  sample of $T$, which admits a $\alpha_f-$Hölder continuous density $f_T$, bounded and bounded away from zero on $[0,1]$.
	Let $\varphi$ be $s-$Hölder continuous with Hölder constant $L_\varphi$. Then, 
	\begin{equation}
		\EE\left[\{ \widehat c_j -\widehat d_j\}^2\varphi(S_j)\right] =  O(n^{-s}+n^{-\alpha_f})  +  
		\left\{ 
		\begin{tabular}{lll}
			$\dfrac{3}{2}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{3,\ldots, n-2 \},$\\
			\\ 	$\dfrac{5}{4}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{2, n-1\},$\\
			\\ $\dfrac{11}{4}\EE\left[\varphi(S_j) \right] $ & \text{if } & $j \in \{1,  n \},$			
		\end{tabular} 
		\right. 
	\end{equation}
	with the constant in $ O(n^{-s}+n^{-\alpha_f})$   depending only on the Hölder exponents, Hölder  constants and the uniform norms  of $f_T$ and $\varphi$. 	
\end{corollary}


%
%\newpage 
%
%
%\begin{remark}
%Let us note that 
%$$
%2F_T\left(\frac{S_{j}+S_{j+1}}{2}  \right) - F_T(S_{j}) - F_T(S_{j+1})
%=  \int_{S_{j}}^{(S_{j}+S_{j+1})/2}f_T(t)dt - \int^{S_{j+1}}_{(S_{j}+S_{j+1})/2}f_T(t)dt
%$$
%and 
%$$
%2F_T\left(\frac{S_{j-1}+S_{j}}{2}  \right) - F_T(S_{j-1}) - F_T(S_{j})
%=  \int_{S_{j-1}}^{(S_{j-1}+S_{j})/2}f_T(t)dt- \int^{S_{j}}_{(S_{j-1}+S_{j})/2}f_T(t)dt  .
%$$
%We deduce that 
%\begin{multline}
%2\left[	F_T\left(\frac{S_{j}+S_{j+1}}{2}  \right) - F_T\left(\frac{S_{j-1}+S_{j}}{2}  \right)\right]=  F_T(S_{j+1}) - F_T(S_{j-1}) \\  +\int_{(S_{j-1}+S_{j})/2}^{(S_{j}+S_{j+1})/2}f_T(t)dt - \int_{S_{j-1}}^{(S_{j-1}+S_{j})/2}f_T(t)dt- \int^{S_{j+1}}_{(S_{j}+S_{j+1})/2}f_T(t)dt\\
%= F_T(S_{j+1}) - F_T(S_{j-1})  + f_T(S_j) \left[\frac{S_{j+1} - S_{j-1}}{2} - \frac{S_{j} - S_{j-1}}{2} - \frac{S_{j+1} - S_{j}}{2} \right]\\
%+ \int_{(S_{j-1}+S_{j})/2}^{(S_{j}+S_{j+1})/2}\{f_T(t)-f(S_j)\}dt - \int_{S_{j-1}}^{(S_{j-1}+S_{j})/2}\{f_T(t)-f(S_j)\}dt- \int^{S_{j+1}}_{(S_{j}+S_{j+1})/2}\{f_T(t)-f(S_j)\}dt\\
%=:F_T(S_{j+1}) - F_T(S_{j-1}) -R_{n,j}.
%\end{multline}
%Since $f_T$ is Lipschitz continuous with constant $C_f$, we have
%$$
%0< R_{n,j} \leq \frac{C_f}{2} \left[ \{S_{j}-S_{j-1}\}^2 + \{S_{j+1}-S_{j}\}^2\right].
%$$ 
%This implies that for the calculations of the moments of $\widehat c_j$, we can only consider the case of uniform $T$. The general case yields similar results up to negligible terms. 
%
%
%\end{remark}




%\bibliographystyle{apalike}
%\bibliography{refs_PW.bib}

%\end{document}
